Statistical Inference on the Hilbert Sphere with Application to Random Densities

The infinite-dimensional Hilbert sphere $S^\infty$ has been widely employed to model density functions and shapes, extending the finite-dimensional counterpart. We consider the Fr\'echet mean as an intrinsic summary of the central tendency of data lying on $S^\infty$. To break a path for sound statistical inference, we derive properties of the Fr\'echet mean on $S^\infty$ by establishing its existence and uniqueness as well as a root-$n$ central limit theorem (CLT) for the sample version, overcoming obstructions from infinite-dimensionality and lack of compactness on $S^\infty$. Intrinsic CLTs for the estimated tangent vectors and covariance operator are also obtained. Asymptotic and bootstrap hypothesis tests for the Fr\'echet mean based on projection and norm are then proposed and are shown to be consistent. The proposed two-sample tests are applied to make inference for daily taxi demand patterns over Manhattan modeled as densities, of which the square roots are analyzed on the Hilbert sphere. Numerical properties of the proposed hypothesis tests which utilize the spherical geometry are studied in the real data application and simulations, where we demonstrate that the tests based on the intrinsic geometry compare favorably to those based on an extrinsic or flat geometry.

==> pre_hans.tex <==
%\newcommand{\Appendix}{\appendix\def\thesection{APPENDIX~\Alph{section}}
%\def\thesubsection{\Alph{section}.\arabic{subsection}}}

\newcommand{\bea}{\begin{eqnarray*}}
\newcommand{\eea}{\end{eqnarray*}}
\newcommand{\be}{\begin{eqnarray}}
\newcommand{\ee}{\end{eqnarray}}
\newcommand{\ed}{\end{document}}
\newcommand{\no}{\noindent}
\newcommand{\et}{\textit{et al. }}
\newcommand{\btab}{\begin{tabular}}
\newcommand{\etab}{\end{tabular}}
\newcommand{\bc}{\begin{center}}
\newcommand{\ec}{\end{center}}
\newcommand{\np}{\newpage}
\newcommand{\la}{\label}
\newcommand{\bi}{\begin{itemize}}
\newcommand{\ei}{\end{itemize}}
\newcommand{\bfi}{\begin{figure}}
\newcommand{\efi}{\end{figure}}
\newcommand{\ben}{\begin{enumerate}}
\newcommand{\een}{\end{enumerate}}
\newcommand{\bdes}{\begin{description}}
\newcommand{\edes}{\end{description}}
\newcommand{\bay}{\begin{array}}
\newcommand{\eay}{\end{array}}
\newcommand{\bs}{\boldsymbol}
\newcommand{\mb}{\boldsymbol}
\newcommand{\nn}{\nonumber}
\newcommand{\sm}{\vspace{.2cm}}

\def\bco{\iffalse}
\def\ci{\cite}
\def\cp{\citep}
\def\eps{\varepsilon}
\def\ep{\epsilon}


\def\ij{_{ij}}
\def\i1{_{i1}}
\def\ik{_{ik}}
\def\ki{_{ki}}
\def\mhf{^{-1/2}}
\def\mo{^{-1}}
\def\ij{_{ij}}
\def\ijk{_{ijk}}
\def\ik{_{ik}}
\def\jj{_{jj}}
\def\jk{_{jk}}
%\def\half{^{1/2}}
\def\refmark{\par\vskip 2mm\noindent\refhg}

\def\gotolimit#1{\mathrel{\mathop{\longrightarrow}\limits^{#1}}}

\def\as{^*}
\newcommand{\hs}{\hspace{0.2cm}}
\def\povr{\buildrel p\over\longrightarrow}
\def\pr{\hbox{pr}}
\def\wh{\widehat}
\def\det{\hbox{det}}
\def\vm{\vspace{-1cm}}

\def\sd{\vspace{-.12in}}
\def\foot#1#2{{\baselineskip=9pt\sevenrm\footnote{$^{#1}$}{#2}}}
\def\nh{\noindent\hangindent=1.5truecm\hangafter=1}

\def\hyi{\hat{y}^{(-i)}}

\newcommand{\lf}{\left}
\newcommand{\R}{\right}
\def\theres{R(\arabic{res})}
\def\povr{\buildrel p\over\longrightarrow}

\def\ss{\subsection*}
\def\sss{\subsubsection*}
\def\sd{\vspace{-.18in}}



\def\me{{\sc Me-spline}}
\def\psp{{\sc P-spline}}
\def\ke{{\sc Kernel}}
\def\cu{{\sc Cubic Spline}}
\def\pa{{\sc Pace 2.9$\,$}}
\def\pae{{\sc Pace-eig}}
\def\quo{{\sc Pace-quo}}
\def\hs{{$\,\,$}}
\def\xe{\zeta}
\def\Xc{X(t)-\mu(t)}
\def\Xd{X^{(1)}(t)-\mu^{(1)}(t)}
\def\Xdd{X^{(1)}(t)}
\def\s2{\sum_{k=1}^\infty\lambda_k\phi_k(t) \phi_k(t)}
\def\s1{\sum_{k=1}^\infty\lambda_k\phi^{(1)}_k(s) \phi_k(t)}
\def\sk{\sum_{k=1}^\infty}
\def\lk{\lambda_k}
\def\pt{\phi_k(t)}
\def\ps{\phi_k(s)}
\def\pt1{\phi^{(1)}_k(t)}
\def\ps1{\phi^{(1)}_k(s)}
\def\de{^{(1)}}

\def\foot#1#2{{\baselineskip=9pt\sevenrm\footnote{$^{#1}$}{#2}}}
\def\nh{\noindent\hangindent=1.5truecm\hangafter=1}

\def\singlespace{\def\baselinestretch{1}\@normalsize}
\def\endsinglespace{}

\newcommand{\single}{\renewcommand{\baselinestretch}{1.2}\normalsize}
\newcommand{\double}{\renewcommand{\baselinestretch}{1.5}\normalsize}


==> preamble.tex <==
%\usepackage{geometry,float}
%\usepackage{bm}
\usepackage{amssymb}
\usepackage{amstext}
\usepackage{graphics}
\usepackage{graphicx}
\usepackage{amsthm}
\usepackage{amsmath}
\usepackage{mathtools}
\usepackage{enumitem}
%\usepackage{pdfpages}
%\usepackage{latexsym}
%\usepackage{lscape}
%\usepackage{color}
%\usepackage{epsfig,epsf,psfrag}
%\usepackage{sectsty}
\usepackage{graphics}
%\usepackage{epsfig}
%\usepackage{html}
\usepackage{rotating}
\usepackage{multirow}
%\usepackage{lscape}
\usepackage[linesnumbered,lined,ruled]{algorithm2e}
\usepackage[colorlinks=true, allcolors=blue, draft=false]{hyperref}
\renewcommand{\itemautorefname}{\hspace{-.4em}}
\renewcommand{\sectionautorefname}{Section}
\renewcommand{\subsectionautorefname}{Subsection}
\newcommand{\Theoremautorefname}{Theorem}
\newcommand{\Remarkautorefname}{Remark}
\newcommand{\Lemmaautorefname}{Lemma}
\newcommand{\Corollaryautorefname}{Corollary}
\newcommand{\Propositionautorefname}{Proposition}
\renewcommand{\algorithmautorefname}{Algorithm}
\renewcommand{\algorithmcflinename}{Line}
\usepackage[authoryear]{natbib}
%\usepackage{slashbox}
%\usepackage[authoryear,super]{natbib}
%\usepackage[mathscr]{eucal}
%\usepackage{lscape}

%\geometry{letterpaper,left=1.2in,right=1.2in,top=1.2in,bottom=1.1in}
%SPACING
\AtBeginDocument{%
  \addtolength\abovedisplayskip{0\baselineskip}%
  \addtolength\belowdisplayskip{0\baselineskip}%
%  \addtolength\abovedisplayshortskip{-0.5\baselineskip}%
%  \addtolength\belowdisplayshortskip{-0.5\baselineskip}%
}


%\bibliographystyle{ims}
\bibpunct{(}{)}{;}{a}{}{,}
\tolerance=500 \allowdisplaybreaks

\graphicspath{{figures/}}

% % % % %Start User Command Definition % % % % %
\newcommand{\code}[1]{\texttt{#1}}
\newcommand{\bla}[1]{\textcolor{black}{#1}}
\newcommand{\blu}[1]{\textcolor{blue}{#1}}
\newcommand{\red}[1]{\textcolor{red}{#1}}
% % % % % End User Command Definition % % % % %

% % % % %Start Math Symbol Definition % % % % %
% Differential operator
\newcommand*{\diff}[2]{\frac{\partial #1}{\partial #2}} 
\AtBeginDocument{\renewcommand{\d}{\mathop{}\!\mathrm{d}}}
% Distributed as symbol
\makeatletter
\newsavebox{\mybox}\newsavebox{\mysim}
\newcommand{\distas}[1]{%
  \savebox{\mybox}{\hbox{\kern3pt$\scriptstyle#1$\kern3pt}}%
  \savebox{\mysim}{\hbox{$\sim$}}%
  \mathbin{\overset{\text{#1}}{\kern\z@\resizebox{\wd\mybox}{\ht\mysim}{$\sim$}}}%
}
\makeatother
% Define as symbol
\newcommand{\defas}{\coloneqq}
% Converge to with mode
\newcommand*{\conv}[1]{\mathrel{\mathop{\longrightarrow}\limits^{#1}}}

\DeclarePairedDelimiterX{\inner}[2]{\langle}{\rangle}{#1, #2}
\DeclarePairedDelimiterX{\Inner}[2]{\langle\langle}{\rangle\rangle}{#1, #2}
\DeclarePairedDelimiterX{\innerp}[2]{\langle}{\rangle_p}{#1, #2}
%\DeclarePairedDelimiterX{\innerR}[2]{\langle}{\rangle_{d}}{#1, #2}
\newcommand{\innerR}[2]{{#1}^T{#2}}

% argmax argmin operators
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

% goes to infinity or zero
\newcommand{\ntoinf}{n \rightarrow \infty}
\newcommand{\deltatozero}{\delta \downarrow 0}
\newcommand{\toinf}{\rightarrow \infty}
\newcommand{\tozero}{\rightarrow 0}
\def\emptyset{\varnothing} % Empty set
\newcommand{\sumjinf}{\sum_{j=1}^\infty}
\newcommand{\sumkinf}{\sum_{k=1}^\infty}
\newcommand{\sumjJ}{\sum_{j=1}^J}
\newcommand{\sumkK}{\sum_{k=1}^K}
\newcommand{\sumin}{\sum_{i=1}^n}

\newcommand{\bbR}{\mathbb{R}}
\newcommand{\bbP}{\mathbb{P}}
\newcommand{\bbG}{\mathbb{G}}
\newcommand{\bbC}{\mathbb{C}}
\newcommand{\bbN}{\mathbb{N}}
\newcommand{\bbZ}{\mathbb{Z}}
\newcommand{\bbH}{\mathbb{H}}
\newcommand{\bbE}{\mathbb{E}}
\newcommand{\bbF}{\mathbb{F}}
\newcommand{\bbM}{\mathbb{M}}

\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\ran}{\mathcal{R}}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\MSPE}{MSPE}
\DeclareMathOperator{\FVE}{FVE}
\DeclareMathOperator{\Var}{Var}
\DeclareMathOperator{\var}{var}
\DeclareMathOperator{\Cov}{Cov}
\DeclareMathOperator{\cov}{cov}
\DeclareMathOperator{\one}{\mathbf{1}}
\DeclareMathOperator{\Exp}{Exp}
\DeclareMathOperator{\Log}{Log}
\DeclareMathOperator{\MSE}{MSE}
\DeclareMathOperator{\Span}{span}
\DeclareMathOperator{\logit}{logit}
\DeclareMathOperator{\expit}{expit}
\DeclareMathOperator{\inj}{inj}
\DeclareMathOperator{\Image}{Im}
\DeclareMathOperator{\Domain}{Dom}

\renewcommand*{\vec}[1]{\mathbf{#1}}
\newcommand*{\bbeta}{\boldsymbol{\beta}}
\newcommand*{\hbbeta}{\hat{\boldsymbol{\beta}}}
\newcommand*{\bmu}{\boldsymbol{\mu}}
\newcommand*{\bxi}{\boldsymbol{\xi}}
\newcommand*{\tbxi}{\tilde{\boldsymbol{\xi}}}
\newcommand*{\bzeta}{\boldsymbol{\zeta}}
\newcommand*{\tbzeta}{\tilde{\boldsymbol{\zeta}}}
\newcommand*{\bphi}{\boldsymbol{\phi}}
\newcommand*{\bPhi}{\boldsymbol{\Phi}}
\newcommand*{\bPsi}{\boldsymbol{\Psi}}
\newcommand*{\hbPhi}{\hat{\boldsymbol{\Phi}}}
\newcommand*{\bSigma}{\boldsymbol{\Sigma}}
\newcommand{\bx}{\vec{x}}
\newcommand{\by}{\vec{y}}
\newcommand{\bY}{\vec{Y}}


\newcommand{\hbeta}{\hat{\beta}}
\newcommand{\hpsi}{\hat{\psi}}
\newcommand{\heta}{\hat{\eta}}
\newcommand{\hsigma}{\hat{\sigma}}
\newcommand{\homega}{\hat{\omega}}
\newcommand{\halpha}{\hat{\alpha}}
\newcommand{\htau}{\hat{\tau}}
\newcommand{\hm}{\hat{m}}
\newcommand{\hmu}{\hat{\mu}}
\newcommand{\ha}{\hat{a}}
\newcommand{\hV}{\hat{V}}
\newcommand{\hU}{\hat{U}}
\newcommand{\hK}{\hat{K}}
\newcommand{\htheta}{\hat{\theta}}
\newcommand{\hSigma}{\hat{\Sigma}}
\newcommand{\hL}{\hat{L}}
\newcommand{\hE}{\hat{E}}
\newcommand{\hF}{\hat{F}}
\newcommand{\hG}{\hat{G}}
\newcommand{\hJ}{\hat{J}}
\newcommand{\hR}{\hat{R}}
\newcommand{\hxi}{\hat{\xi}}
\newcommand{\hLambda}{\hat{\Lambda}}
\newcommand{\hlambda}{\hat{\lambda}}
\newcommand{\hphi}{\hat{\phi}}
\newcommand{\hbphi}{\hat{\bphi}}
\newcommand{\hy}{\hat{y}}
\newcommand{\hX}{\hat{X}}
\newcommand{\hFVE}{\widehat{\FVE}}
\newcommand{\hnu}{\hat{\nu}}

\newcommand{\barX}{\bar{X}}
\newcommand{\barx}{\bar{x}}
\newcommand{\bary}{\bar{y}}
\newcommand{\barY}{\bar{Y}}
\newcommand{\barV}{\bar{V}}

\newcommand{\tmu}{\tilde{\mu}}
\newcommand{\ttheta}{\tilde{\theta}}
\newcommand{\teta}{\tilde{\eta}}
\newcommand{\tbeta}{\tilde{\beta}}
\newcommand{\ts}{\tilde{s}}
\newcommand{\tL}{\tilde{L}}
\newcommand{\tE}{\tilde{\E}}
\newcommand{\tV}{\tilde{V}}
\newcommand{\tX}{\tilde{X}}
\newcommand{\tY}{\tilde{Y}}
\newcommand{\tZ}{\tilde{Z}}
\newcommand{\tD}{\tilde{D}}
\newcommand{\tG}{\tilde{G}}
\newcommand{\tM}{\tilde{M}}
\newcommand{\tXi}{\tX_i}
\newcommand{\tXj}{\tX_j}

\newcommand{\vA}{\vec{A}}
\newcommand{\vU}{\vec{U}}
\newcommand{\vV}{\vec{V}}
\newcommand{\vu}{\vec{u}}
\newcommand{\vv}{\vec{v}}
\newcommand{\vy}{\vec{y}}
\newcommand{\vt}{\vec{t}}

\newcommand*{\cA}{\mathcal{A}}
\newcommand*{\cB}{\mathcal{B}}
\newcommand*{\cC}{\mathcal{C}}
\newcommand*{\cD}{\mathcal{D}}
\newcommand*{\cE}{\mathcal{E}}
\newcommand*{\cF}{\mathcal{F}}
\newcommand*{\cG}{\mathcal{G}}
\newcommand*{\cH}{\mathcal{H}}
\newcommand*{\cI}{\mathcal{I}}
\newcommand*{\cJ}{\mathcal{J}}
\newcommand*{\cK}{\mathcal{K}}
\newcommand*{\cL}{\mathcal{L}}
\newcommand*{\cM}{\mathcal{M}}
\newcommand*{\cN}{\mathcal{N}}
\newcommand*{\cO}{\mathcal{O}}
\newcommand*{\cP}{\mathcal{P}}
\newcommand*{\cQ}{\mathcal{Q}}
\newcommand*{\cR}{\mathcal{R}}
\newcommand*{\cS}{\mathcal{S}}
\newcommand*{\cT}{\mathcal{T}}
\newcommand*{\cU}{\mathcal{U}}
\newcommand*{\cV}{\mathcal{V}}
\newcommand*{\cW}{\mathcal{W}}
\newcommand*{\cX}{\mathcal{X}}
\newcommand*{\cY}{\mathcal{Y}}
\newcommand*{\cZ}{\mathcal{Z}}


\newcommand*{\Xic}{X_i^c}
\newcommand*{\half}{\frac{1}{2}}
\newcommand*{\tohalf}{^{\frac{1}{2}}}
\newcommand*{\inv}{^{-1}}
% % % % %End Math Symbol Definition % % % % %

\usepackage{amsthm}
\theoremstyle{compact.definition}
%\newtheorem*{axm}{Axm}
%\newtheorem*{defn}{Def}
%\newtheorem*{thm}{Thm}
%\newtheorem*{lem}{Lem}
%\newtheorem*{cor}{Crl}
%\newtheorem*{prop}{Prop}
%\newtheorem*{eg}{Eg}
\newtheorem{Theorem}{Theorem}
\newtheorem{Lemma}{Lemma}
\newtheorem{Corollary}{Corollary}
\newtheorem{Proposition}{Proposition}%\renewcommand{\qedsymbol}{} % Remove QED symbol

\makeatletter
\def\th@newremark{\th@remark\thm@headfont{\bfseries}} % Bold the remark title
\makeatletter
\theoremstyle{newremark}
\newtheorem{Remark}{Remark}

\theoremstyle{compact.remark}
\newtheorem*{prf}{Proof}
\newtheorem*{note}{Note}
\newtheorem*{rmk}{Remark}

% PAPER SPECIFIC
\newcommand{\jonetoinf}{_{j = 1}^\infty}
\newcommand{\konetoinf}{_{k = 1}^\infty}
\newcommand{\nonetoinf}{_{n = 1}^\infty}
\newcommand{\jonetoJ}{_{j = 1}^J}
\newcommand{\limktoinf}{\lim_{k\toinf}}
\newcommand{\limntoinf}{\lim_{n\toinf}}
\newcommand{\pinf}{p_{\infty}}
\newcommand{\Sinf}{\cS^{\infty}}
\newcommand{\normp}[1]{\left\lVert#1\right\rVert_p}
\newcommand{\Tmut}{T_{\mu(t)}} 
\newcommand{\TmutS}{T_{\mu(t)}\Sinf}
\newcommand{\Thmu}{T_{\hmu}} 
\newcommand{\Thmut}{T_{\hmu(t)}} 
\newcommand{\ThmutS}{T_{\hmu(t)}\Sinf}
\newcommand{\hcG}{\hat{\cG}}
\newcommand{\hcV}{\hat{\cV}}

\newcommand{\quadas}{\quad \text{a.s.}}
\newcommand{\oneovern}{\frac{1}{n}}
\newcommand{\oneoverrootn}{\frac{1}{\sqrt{n}}}
\newcommand{\noverlogn}{\frac{n}{\log n}}
\newcommand{\lognovern}{\frac{\log n}{n}}
\newcommand{\sqrtn}{\sqrt{n}}

\newcommand{\Tmu}{T_{\mu}\Sinf}
\newcommand{\logmu}{\log_{\mu}}
\newcommand{\logmut}{\log_{\mu(t)}}
\newcommand{\loghmu}{\log_{\hmu}}
\newcommand{\loghmut}{\log_{\hmu(t)}}
\newcommand{\expmu}{\exp_{\mu}}
\newcommand{\expmut}{\exp_{\mu(t)}}
\newcommand{\exphmu}{\exp_{\hmu}}
\newcommand{\exphmut}{\exp_{\hmu(t)}}
\newcommand{\hmuMs}{{\hmu_\cMd(s)}}
\newcommand{\intcT}{\int_\cT}
\newcommand{\lambdamin}{\lambda_{\min}}
\newcommand{\inft}{\inf_{t \in \cT}}
\newcommand{\supt}{\sup_{t \in \cT}}
\newcommand{\supp}{\sup_{p \in \Sinf}}
\newcommand{\supttss}{\sup_{t_1,t_2\in \cT,\, s_1,s_2\in\cS}}
\newcommand{\supj}{\sup_{j\ge 1}}
\newcommand{\infpSinf}{\inf_{p\in\Sinf}}

\newcommand{\tinT}{t \in \cT}
\newcommand{\sinS}{s \in \cS}
\newcommand{\hinH}{h \in \cH}
\newcommand{\pinSInf}{p \in \Sinf}

\newcommand{\abs}[1]{\left\lvert#1\right\rvert}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\normE}[1]{\left\lVert#1\right\rVert_{\bbE}}
\newcommand{\normEs}[1]{\left\lVert#1\right\rVert_{\bbE^*}}
\newcommand{\normF}[1]{\left\lVert#1\right\rVert_{\bbF}}
\newcommand{\normshort}[1]{\lVert#1\rVert}
\newcommand{\Norm}[1]{{\left\vert\kern-0.25ex\left\vert\kern-0.25ex\left\vert #1 \right\vert\kern-0.25ex\right\vert\kern-0.25ex\right\vert}}
%\newcommand{\Norm}[1]{\left\vertiii #1 \right\vertiii}
%\newcommand{\dtau}{d_{\tau}}
\newcommand{\rhotau}{\rho_{\tau}}
\newcommand{\rhoupsilon}{\rho_{\upsilon}}
\newcommand{\tnu}{\tilde{\nu}}

\newcommand{\barcB}{\bar{\cB}}
\newcommand{\bnqc}{\mathbf{n}_{q_c}}
\newcommand{\tq}{\tilde{q}}
\newcommand{\sinSinf}{s \in \Sinf}
\newcommand{\suppSinf}{\sup_{p \in \Sinf}}
\newcommand{\inftT}{\inf_{t \in \cT}}
\newcommand{\suptT}{\sup_{t \in \cT}}
\newcommand{\suphH}{\sup_{h \in \cH}}
\newcommand{\infpmuteps}{\inf_{\rho(p, \mu(t)) \ge \epsilon}}
\newcommand{\infpmuzeps}{\inf_{\substack{\norm{p} = 1 \\ \rho(p, \mu(0)) \ge \epsilon}}}
\newcommand{\infpmuzbeps}{\inf_{\substack{\norm{p\le 1} \\ \rho(p, \mu(0)) \ge \epsilon}}}

\newcommand{\Pij}{\Pi_{I_{j}}}
\newcommand{\Pijp}{\Pi_{I_{j}^\perp}}
\newcommand{\mutau}{\mu_{\tau}}
\newcommand{\Xtau}{X_{\tau}}
\newcommand{\xitau}{x_{i,\tau}}
\newcommand{\hmutau}{\hmu_{\tau}}
\newcommand{\psitau}{\psi_{\tau}}
\newcommand{\Psitau}{\Psi_{\tau}}
\newcommand{\Psintau}{\Psi_{n,\tau}}
\newcommand{\xiupsilont}{x_{i,\upsilon_t}}
\newcommand{\Xupsilont}{X_{\upsilon_t}}
\newcommand{\muupsilont}{\mu_{\upsilon_t}}
\newcommand{\psiupsilont}{\psi_{\upsilon_t}}
\newcommand{\Psiupsilont}{\Psi_{\upsilon_t}}
\newcommand{\Psinupsilont}{\Psi_{n,\upsilon_t}}
\newcommand{\hmuHS}{\hmu_{\text{I}}}
\newcommand{\hphiJHS}{\hphi_{J,\text{I}}}
\newcommand{\hxiJHS}{\hxi_{J,\text{I}}}
\newcommand{\hlambdaJHS}{\hlambda_{J,\text{I}}}
\newcommand{\hXJHS}{\hX_{J,\text{I}}}
\newcommand{\hmuL}{\hmu_{\text{E}}}
\newcommand{\hphiJL}{\hphi_{J,\text{E}}}
\newcommand{\hxiJL}{\hxi_{J,\text{E}}}
\newcommand{\hlambdaJL}{\hlambda_{J,\text{E}}}
\newcommand{\hXJL}{\hX_{J,\text{E}}}
